Consistency Purification: Effective and Efficient Diffusion Purification towards Certified Robustness

Diffusion Purification, purifying noised images with diffusion models, has been widely used for enhancing certified robustness via randomized smoothing. However, existing frameworks often grapple with the balance between efficiency and effectiveness. While the Denoising Diffusion Probabilistic Model (DDPM) offers an efficient single-step purification, it falls short in ensuring purified images reside on the data manifold. Conversely, the Stochastic Diffusion Model effectively places purified images on the data manifold but demands solving cumbersome stochastic differential equations, while its derivative, the Probability Flow Ordinary Differential Equation (PF-ODE), though solving simpler ordinary differential equations, still requires multiple computational steps. In this work, we demonstrated that an ideal purification pipeline should generate the purified images on the data manifold that are as much semantically aligned to the original images for effectiveness in one step for efficiency. Therefore, we introduced Consistency Purification, an efficiency-effectiveness Pareto superior purifier compared to the previous work. Consistency Purification employs the consistency model, a one-step generative model distilled from PF-ODE, thus can generate on-manifold purified images with a single network evaluation. However, the consistency model is designed not for purification thus it does not inherently ensure semantic alignment between purified and original images. To resolve this issue, we further refine it through Consistency Fine-tuning with LPIPS loss, which enables more aligned semantic meaning while keeping the purified images on data manifold. Our comprehensive experiments demonstrate that our Consistency Purification framework achieves state-of the-art certified robustness and efficiency compared to baseline methods.

==> section/3method.tex <==
\section{Theoretical Analysis}
% \kun{Below are just some initial thoughts, the roadmap for showing ODE > one-step is that ODE has some attraction properties, and we want to show that each training sample has some attraction region, and we use a two sample toy example to show the idea}

% \zz{Please formally introduce the framework here.}

Compared with \cite{carlini2022certified, xiao2022densepure}, our method has two main advantages:
\begin{enumerate}
    \item (Recovery by PF ODE trajectory) We propose utilizing the \ref{probODE} trajectory for denoising, rather than relying on the \ref{onestepdenoiser} or the \ref{reverseSDE}. Under mild conditions, given a noisy sample $\rvx_t$ with corresponding timestep $t$, there exists a unique ODE trajectory that $\rvx_t$ should lie on. The clean sample $\rvx_0$, located at the end of this trajectory when $t = 0$, serves as the purified output in our framework. While the \ref{onestepdenoiser} is fast and deterministic, it generates the mean of the posterior data distribution given $(\rvx_t, t)$, which does not necessarily locate on the data manifold and may exhibit ambiguity during classification. On the other hand, while \ref{reverseSDE} guarantees the generated example to be on data manifold, the location is stochastic and may not be aligned with the original sample in the semantic sense, which is why \cite{xiao2022densepure} has to use the ``majority vote" strategy to derandomize. Our framework resolves the issues in both methods. It leverages the direct mapping from $(\rvx_t, t)$ to $(\rvx_0, 0)$ in the ODE trajectory for denoising in just one step, while having the purified sample $\rvx_0$ lying on the data manifold.

    \item (Finetuning by semantic alignment) We propose finetuning the consistency model to enhance the semantic consistency of the denoised sample. The PF ODE trajectory does not ensure that samples lying on the same path maintain identical semantic meaning. As a result, the purified sample obtained through the PF ODE trajectory may not retain the original class of the noisy input. To address this, we finetune the consistency model using LPIPS loss to minimize the perceptual difference between the original and purified samples. This approach ensures that the purified sample captures the semantic meaning of the original without being too constrained to the exact data point, which could disrupt consistency model's structure and degrade recovery performance.
\end{enumerate}

In this section, we elaborate on the theoretical explanations of why Consistency Purification can improve the purification performance in terms of certified accuracy and certified robustness over \cite{carlini2022certified, xiao2022densepure}. 

% The recovery by PF ODE has the advantage of getting a purified sample that is ``on-manifold''. In a simplified case where the original distribution is a weighted sum of dirac delta functions made of the training samples \cite{} (EDM), the ODE can recover a noisy sample sufficiently close to a training sample under certain conditions, but the one-step method will not recover to a training sample with probability one. 

% We formalize the above argument in proposition 1, where we need to first introduce the \emph{Posterior Mean Mapping} $\Phi: \mathbb{R}^d \rightarrow \mathbb{R}^d$ and \emph{Monotonic Posterior Neighborhood} (MPN).

% \begin{definition} \label{defn:post_mean_map} (Posterior Mean Mapping and Monotonic Posterior Neighborhood)\\
%     For any given noisy sample $\boldsymbol{x}$, noise variance $\sigma^2$, and training samples $\{\boldsymbol{y}_i\}_{i=1}^{N}$, we denote the Posterior Mean Mapping as
%     \begin{equation} \label{eq:PMM}
%         \Phi(\boldsymbol{x}; \sigma) :=  \frac{\sum_i \mathcal{N}(\boldsymbol{x};\boldsymbol{y}_i, \sigma^2 I) \boldsymbol{y}_i}{\sum_i \mathcal{N}(\boldsymbol{x};\boldsymbol{y}_i, \sigma^2 I)}. 
%     \end{equation}
%     Then suppose $\sigma^2$ is the noise variance at the \emph{reverse starting time}, we define the Monotonic Posterior Neighborhood of sample $\boldsymbol{y}_i$ as
%     \begin{equation} \label{eq:MPN}
%         \mathcal{S}_{i} := \left \{\boldsymbol{x} \bigg | \frac{\mathcal{N}(\boldsymbol{x};\boldsymbol{y}_i, \sigma^2 I) \| \boldsymbol{y}_i - \boldsymbol{x} \|_2}{\sum_i \mathcal{N}(\boldsymbol{x};\boldsymbol{y}_i, \sigma^2 I)} \geq \|  \Phi(\boldsymbol{x}) - \boldsymbol{x} \|_2 \right \}.
%     \end{equation}
% \end{definition}

% \begin{proposition} (Attraction Effect in the MPN) \\
%     Given the noise variance $\sigma^2$, and training samples $\{\boldsymbol{y}_i\}_{i=1}^{N}$, for any noisy sample in $\mathcal{S}_{i}$, the ODE will eventually recover $\boldsymbol{y}_i$.
% \end{proposition}

% \begin{proof} (Sketch) 
%     Let's take a discretized view to the ODE, which is analogous to a gradient descent type of update. At a given snapshot $t \in [T]$ (since we discretize the process, the time scale is now similar to DDPM), we will be given a fixed $\sigma_t$ according to the noise scale and a corresponding noisy sample $\boldsymbol{x}_t$, then we can compute the posterior mean at this snapshot, which is $\Phi(\boldsymbol{x}_t; \sigma_t)$, and we can do a gradient step to get the previous snapshot's sample $\boldsymbol{x}_{t-1} = (1-\eta_t)\boldsymbol{x} + \eta_t \Phi(\boldsymbol{x}_t; \sigma_t)$. From the definition of MPN, we know that there exists a sufficiently small $\eta_t > 0$ such that $\|\boldsymbol{x}_{t-1} - \boldsymbol{y}_i\|_2 < \|\boldsymbol{x}_{t-1} - \boldsymbol{y}_i\|_2$. 
% \end{proof}

As demonstrated in \cite{Song2021ICLR}, \ref{probODE} maintains the marginal distribution of \ref{reverseSDE}, thereby establishing a deterministic mapping between the noisy distribution \(\vx_t\) and the data distribution \(\vx_0\). In other words, \ref{probODE} guarantees that the purified sample lies on the data manifold, unlike \ref{onestepdenoiser}, which lacks this assurance. Additionally, \ref{probODE} is deterministic, eliminating the overhead of majority voting required when using \ref{reverseSDE} as a purifier. The consistency model, which reduces ODE solving to a one-step mapping, further ensures purification has the same efficiency as \ref{onestepdenoiser} while keeping the on-manifold property.

We present here a simple one dimensional example for illustration.

% Below we present a toy example showing why it is important to have a purified sample on the data manifold, i.e., the advantage of ODE trajectory over posterior mean for adversarial purification. 

\begin{example}
   Consider a one-dimensional space with a data set consisting of two samples \(\{\vy_1, \vy_2\}\), where \(\vy_1 = 1\) and \(\vy_2 = -1\). The distribution can be represented as a mixture of Dirac delta distributions: $p_{\text{data}}(\vx) = \frac{1}{2}\left(\delta(\vx-\vy_1)+ \delta(\vx-\vy_2
    )\right)$. By setting $s(t)=1$ and $\sigma(t)=t$ in \ref{perturbation-kernel}, the distribution at time \(t\) becomes: $p_t(\vx)= \frac{1}{2t\sqrt{2\pi}} \big( e^{-\frac{1}{2}\left(\frac{\vx-1}{t}\right)^2}+  e^{-\frac{1}{2}\left(\frac{\vx+1}{t}\right)^2}\big)$. Then
    \begin{align*}
       \textstyle \frac{\mathrm{d} \log p_t(\vx) }{\mathrm{d} \vx} ~&~\textstyle= \frac{-\left(\frac{\vx-1}{t}\right)e^{-\frac{1}{2}\left(\frac{\vx-1}{t^2}\right)^2}-\left(\frac{\vx+1}{t}\right)e^{-\frac{1}{2}\left(\frac{\vx+1}{t^2}\right)^2}}{2t\sqrt{2\pi} p_t(\vx)}\\
       ~&\textstyle=~ -\frac{\vx}{t^2} + \frac{e^{-\frac{1}{2}\left(\frac{\vx-1}{t}\right)^2}-  e^{-\frac{1}{2}\left(\frac{\vx+1}{t}\right)^2}}{e^{-\frac{1}{2}\left(\frac{\vx-1}{t}\right)^2}+  e^{-\frac{1}{2}\left(\frac{\vx+1}{t}\right)^2}}.
    \end{align*}
From the derivative formula \(\frac{\mathrm{d} \log p_t(\vx)}{\mathrm{d} \vx}\), it's evident that \(\vx = 0\) is an equilibrium point, and the right-hand side expression is Lipschitz continuous around \(\vx = 0\) by L'Hôpital's rule. Thus, according to the Picard-Lindelöf theorem, any trajectory starting on either side of \(\vx = 0\) will not cross this point. As \ref{probODE} drives \(p_t(\vx)\) closer to the Dirac delta distribution \(p_{\text{data}}(\vx)\) as \(t\) approaches zero, any initial point on positive/negative side of \(\vx = 0\) will eventually approach \(1\) or \(-1\), i.e., the data manifold. Furthermore, in this example, \ref{probODE} generates not only a purified sample on the data manifold but also closest to the noisy sample. This property is desirable as it establishes a relatively large "robust" neighborhood around each true data point, which implies high certified robustness and a significant certified radius, which will be further discussed later. With the consistency model, we do not need to solve the ODE but rather directly map the noisy sample to either $1/-1$ depending on its location relative to $\vx=0$.


For comparison, given any $\vx$ and $t$, the \ref{onestepdenoiser} will output a posterior mean that is
\begin{align*}
  \textstyle \frac{e^{-\frac{1}{2}\left(\frac{\vx-1}{t}\right)^2}-  e^{-\frac{1}{2}\left(\frac{\vx+1}{t}\right)^2}}{ e^{-\frac{1}{2}\left(\frac{\vx-1}{t}\right)^2}+  e^{-\frac{1}{2}\left(\frac{\vx+1}{t}\right)^2}} = \textstyle \frac{e^{\frac{2\vx}{t^2}}-1}{e^{\frac{2\vx}{t^2}}+1}.
\end{align*}
The posterior mean will be near \(1\) or \(-1\) only when \(t\) is sufficiently small compared to \(\|\vx\|\). Otherwise, it deviates from the data manifold. In the case when \(t\) is large, the posterior mean will be close to zero, locating in an ambiguous classification region. In adversarial purification \cite{carlini2022certified, xiao2022densepure, nie2022diffusion}, we typically select \(t\) based on the variance of the noise added to the data sample rather than using an very small \(t\). This practice helps avoid significant deviations in the posterior mean estimation due to the imperfect estimation of score/noise. With a very small \(t\), even a slight bias in score/noise estimation can lead to a substantial deviation, resulting in a denoised sample even farther from the data manifold represented by \(p_{\text{data}}(\vx)\).

% Given \((\vx, t)\), it is evident that although \ref{reverseSDE} can produce a purified sample on the manifold, the position of this sample is random:
% \begin{align*}
% \textstyle P(\vx_0 = \mathbf{y}_1 \mid \vx, t) = \frac{e^{-\frac{1}{2}\left( \frac{\vx - 1}{t} \right)^2}}{e^{-\frac{1}{2}\left( \frac{\vx - 1}{t} \right)^2} + e^{-\frac{1}{2}\left( \frac{\vx + 1}{t} \right)^2}}, \quad P(\vx_0 = \mathbf{y}_2 \mid \vx, t) = \frac{e^{-\frac{1}{2}\left( \frac{\vx + 1}{t} \right)^2}}{e^{-\frac{1}{2}\left( \frac{\vx - 1}{t} \right)^2} + e^{-\frac{1}{2}\left( \frac{\vx + 1}{t} \right)^2}}.
% \end{align*}
% Although multiple runs of \ref{reverseSDE} can yield a set of samples for a majority vote to classify, this requires several expensive rounds of SDE solving and still suffers from random errors.

% However, the \ref{EDMODE} does not have this problem because we are solving an ordinary equation function. As long as the discretization step is sufficiently small in the numerical solver, we will end up with a small neighbourhood of the data manifold even if the score/noise estimation has a little bias.

% This property of \ref{EDMODE} is super-beneficial especially when the decision boundary of the classifier is only clear around the data manifold indicated by $p_{\text{data}}(\vx)$ while being ambiguous elsewhere (e.g., the classifier is trained with data from the data manifold), where a denoised sample cannot be recognized correctly by a classifier when lying far away from the data manifold.
\end{example}

% \zz{if we want a graph like this, we might also need to add a case where $\vx_t$ first move right towards 0 and then move left back to -1}
% \begin{figure}[h!]
%     \centering
% \includegraphics[width=\linewidth]{reverse_example.png}
%     \caption{The illustration of the reverse processes in ODE and 1-Step in Example 1.}
%     \label{fig:reverse_example}
% \end{figure}

\zz{We can draw a more general graph to show that one-step DDPM does not denoise the noised samples to the data manifold while ODE can}

Though the consistency model enjoys both on-manifold property and one-step efficiency, it does not guarantee that the purified sample has the same semantic meaning as the original sample. This is because the derivation of \ref{probODE} only guarantees a mapping between noisy distribution and data distribution, which is sufficient for generation, but not enough for denoising purposes. 
\zz{show graph here that ODE could generate a sample with different semantic meaning}

% In the following, we first characterize what property the mapping between the noisy distribution and the data distribution should have for denoising purpose. For convenience we assume that the data distribution follows a 
% discrete distribution with data points $\{\vx_1, \vx_2, \ldots, \vx_n\}$ with probability $p(\vx_i) = \frac{1}{n}$. For either adversarial purification or certified robustness, it is generally desired that if a noisy sample lies within the neighbourhood of a data point, a purifier should output the corresponding data point as the purified sample. The reason are as follows: (1) for adversarial purification, the adversarial sample is typically close to the true sample and a purifier with the above property should be sufficient to successfully denoise such a adversarial sample, (2) for certified robustness, the most common way to establish the certified robustness radius is via randomized smoothing \cite{Cohen2019Iconsistency modelL}, where we add Gaussian noises to a data point to generate noisy samples, then we use a purifier to denoise the noisy samples and classify them, the certified robustness radius depend on probabilities of the true class and other classes. In principle, the larger the differences between the probabilities, the larger the certified robustness radius. Due to the Gaussian distribution property, most probability is assigned to noisy samples near to the data point, the purifier satisfying the above property should be able successfully denoise all such noisy sample, and thus lead to a large certified robustness radius.

In the following, we first characterize the desired properties of the mapping between the noisy and data distributions for denoising purposes. For simplicity, we will assume that the data distribution is discrete, consisting of data points \(\{\vx_1, \vx_2, \ldots, \vx_n\}\) with probability \( p(\vx_i) = \frac{1}{n} \). 

In general, for desirable certified robustness, if a noisy sample lies within the near neighborhood of a certain data point, a purifier should output that data point as the purified sample. On one hand, 
% except for the extreme case, closer samples to the data point tend to have more similar semantic meanings. \zz{fair to say?} 
most attacks and noises have small magnitudes compared with the pairwise distances between data points, and thus if we were to do the purification and recover a purified sample on the data manifold, the data sample closest to the noisy sample would be the correct option.
On the other hand, in certified robustness, the most common method for establishing the certified robustness radius is via randomized smoothing \cite{Cohen2019ICML}, which adds Gaussian noise to a data point to generate augmented noisy samples. A purifier then denoises these augmented samples to get augmented purified samples and classifies them. The certified robustness radius is positive when the true (original sample's) class has the highest probability, and the radius grows with the probability differences between the true and other classes. Due to Gaussian distribution, most probability is assigned to augmented noisy samples near the data point we want to purify. A purifier satisfying the above property should denoise all such augmented noisy samples to the original sample, thus achieving a high probability for the true class, leading to a large certified robustness radius.

We formally define the above property as follows. 
\begin{definition}
    Given a data distribution \( p(\vx_i) = \frac{1}{n} \), a purifier that maps any noisy sample to the nearest (L2 distance) true sample with probability one is referred to as a ``nearest-neighbor purifier".
\end{definition}

Although it is theoretically feasible to compute the distance from a noisy sample to all data points in order to identify the nearest neighbor, this approach is often impractical due to the curse of dimensionality. Rather than seeking an exact nearest-neighbor purifier, we define the characteristics that a purifier should possess to function as an approximate ``nearest-neighbor purifier." This definition leverages the subsequent definition.

\begin{definition}
    Given a purifier $f$ mapping from the noisy distribution $p_t$ to the data distribution $p$, we define ``transport" under $f$ from $p_t$ to $p$ as $D_f(p_t, p): =\int \|\vx_t -f(\vx_t)\| \cdot  p_t(\vx_t) d \vx_t$. We also define ``partial transport" under radius $r$ as $D_f^r(p_t, p): =\int_{\|\vx_t -f(\vx_t)\| < r} \|\vx_t -f(\vx_t)\| \cdot  p_t(\vx_t) d \vx_t$. 
\end{definition}

Intuitively, transport measures the distance between the noisy and purified samples, which should be small by an effective (approximate) nearest-neighbor purifier. There exists a well-established theoretical framework regarding optimal transport, which seeks to minimize the transport between distributions $p_t$ and $p$, as discussed in works such as \cite{peyre2019computational}. Although the nearest-neighbor purifier is not exactly equivalent to the optimal transport purifier due to the transport's dependency on the specific distributions $p$ and $p_t$, we demonstrate that under mild assumptions, a purifier achieving lower transport tends to approximate the nearest-neighbor purifier more closely.

We assume that for a given data point $\vx$, the conditional distribution of noisy samples $p_t(\vx_t | \vx)$, resulting from noise addition, is concentrated around $\vx$. This assumption is justifiable given scenarios like adversarial attacks and randomized smoothing, where a significant deviation of $\vx_t$ from $\vx$ would undermine the rationale for considering the perturbations as relevant or representative noise. Below, we quantify this assumption and present our main theorem.

\begin{theorem}\label{thm:tranport}
    Suppose that the distance between any two data points from different classes is at least $d$. Let $p_r$ be the probability of the noisy samples $\vx_t$ generated by adding noises to a data point $\vx$ are within the $r$ radius of $\vx$, i.e., $p_r:=P(\|\vx_t- \vx\| < r)$. Let $f^*, f$ be the nearest-neighbour purifier and user-trained purifier respectively, then with probability at least $1-q$ where $q=\min_{r\le d/2} q_r$ with $q_r:=\left\{\frac{D_{f}^r(p_t, p)-D_{f^*}^r(p_t, p)}{p_r\cdot(d-2r)}, \frac{D_{f}^r(p_t, p)}{p_r\cdot (d-r)}\right\}$, $f$ will purify a noisy sample $\vx_t$ conditioned on $\|\vx_t- \vx\| < r$ to its nearest data point.
\end{theorem}

\begin{proof}
    Let $q_r$ be the proportion of noisy samples $\vx_t$ conditioned on $\|\vx_t- \vx\| < r$ such that $f(\vx_t) \neq  \vx$. On one hand,
    \begin{align*}
        \textstyle D_f^r(p_t, p) - D_{f^*}^r(p_t, p) &\textstyle~= \int_{f(\vx_t) = \vx} \|\vx_t -f(\vx_t)\| d\vx_t + \int_{f(\vx_t) \neq \vx} \|\vx_t -f(\vx_t)\| d\vx_t\\
        &\textstyle ~=  \int_{f(\vx_t) = \vx} \|\vx_t -f(\vx_t)\| d\vx_t - \int_{f(\vx_t) = \vx} \|\vx_t -f^*(\vx_t)\| d\vx_t \\
        & \textstyle \quad + \int_{f(\vx_t) \neq \vx} \|\vx_t -f(\vx_t)\| d\vx_t - \int_{f(\vx_t) \neq \vx} \|\vx_t -f^*(\vx_t)\| d\vx_t\\
        &\textstyle ~\ge q_r \cdot p_r\cdot   \left(d-2r\right).
    \end{align*}
In other words, $q_r\le \frac{D_{f}^r(p_t, p)-D_{f^*}^r(p_t, p)}{p_r\cdot(d-2r)}$. On the other hand, by Markov's inequality, 
\begin{align*}
    \textstyle q_r = P\left(\|\vx_t -f(\vx_t)\| > d-r \mid \|\vx_t- \vx\| < r\right) \le \frac{E[\|\vx_t -f(\vx_t)\|\mid \|\vx_t- \vx\| < r]}{d-r} = \frac{D_{f}^r(p_t, p)}{p_r\cdot (d-r)}.
\end{align*}
The final probability $1-q$ is taken over the best one over all $r$.
\end{proof}

\begin{remark}
    In Theorem \ref{thm:tranport}, $d$ is the minimum distance between any two data points from different classes, which inherently can be significantly larger than the minimum distance between any two data points, making our theorem stronger. $p_r$ can be either estimated via numerical simulation or calculated from the commonly-seen distribution, like chi-square distribution when the noise follows Gaussian distribution. The probability $1-q$ is large either when the difference between the transports of our purifier and the nearest-neighbour purifier is small or when the transport of our purifier itself is small. Note that when $r$ grows, $p_r$ becomes larger while $d-2r/d-r$ becomes smaller, so the best probability is achieved at some medium $r$.
\end{remark}

From the discussion above, a purifier with small transport generally indicates enhanced semantic alignment and certified robustness. Nevertheless, the ODE trajectory generated by consistency does not inherently ensure this property. To alleviate this issue, we propose finetuning the consistency model by minimizing the LPIPS loss between the purified and original samples. This approach is based on the premise that perturbations in randomized smoothing are typically minor, keeping noisy samples close to the original. By aligning the purified sample more closely with the original, it also approximates the noisy sample better. The choice of LPIPS loss over L-2 loss avoids overly stringent constraints that could disrupt the ODE trajectory, potentially displacing the purified sample from the data manifold. Additionally, we choose to minimize the LPIPS loss between the purified and original samples because we only want to align the purified sample with a clean semantic pattern.




% Further, the following theorem characterize the condition for a mapping between the noisy distribution and the data distribution to be a ``nearest-neighbor purifier".
% \begin{theorem}
%     Given a data distribution $p$ such that \( p(\vx_i) = \frac{1}{n} \) and a noisy distribution $\hat p$ generated by adding any form of noise distribution to $p$. If a mapping $d: \hat p\rightarrow p$ establish an optimal transport between $p$ and $\hat p$, then $d$ serves as a ``nearest-neighbor purifier".
% \end{theorem}
% \begin{proof}
%     If there is a set of noisy samples with non-zero probability that $d$ does not map to their nearest true samples, then there must exist another set of noisy 
% \end{proof}


% \begin{assumption} \label{asm:inter_class_distance} (\textbf{Inter-class Distance Assumption})
%      Suppose the distance between any two data points from different classes is at least \(d = 2r\). 
% \end{assumption}
% This assumption is realistic when we consider the original distribution to be a sum of Dirac-delta functions.

% \begin{assumption} \label{asm:OT_ODE_prufication_rate} (\textbf{Purification Success Rate for OT-ODE})
%     For a given dataset $\mathcal{D}$, and a noise variance at the final time step $\sigma^2_t$, $p_{\mathcal{D}, \sigma^2_t}$ is the successful purification rate of the corresponding OT-ODE from $p_t$ to $p_0$.
% \end{assumption}
% This assumption is also realistic since the OT-ODE will have an inevitable failed purification rate of $1 - p_{\mathcal{D}, \sigma^2_t}$ due to the noise at $t$ being too large that noisy samples gets closer to other samples than the original one.

% Below we show that ODE will bring most adversarial samples to the true neighbourhood using similar techniques as in \cite{nie2022diffusion}
% \begin{theorem} \label{thm:non_OT_ODE_purification_prob} (\textbf{Purification Success Rate for ODE mappings}) Under \cref{asm:inter_class_distance}, \ref{asm:OT_ODE_prufication_rate}, and suppose the denoiser maps the noised sample to the data manifold, and the induced transport cost by this mapping is \((1+q)\) of the optimal transport (OT-ODE) cost (denoted by $C_{OT}$) between the noisy and original distributions ($p_t$ to $p_0$). Then the purification success rate of this denoiser is lower bounded by $1 - p_{\mathcal{D}, \sigma^2_t} - h(q;\sigma^2_t)$, where
% \begin{equation}
%     h(q;\sigma^2_t) := \int_{0}^{d_q} p(\|x_t - x_0\| = r - s; \sigma_t^2) d s,
% \end{equation}
% and $\int_{0}^{d_q} p(\|x_t - x_0\| = r - s; \sigma^2) (2 s) d s = q \cdot C_{OT}$.
% \end{theorem}
% \begin{proof} (Sketch)
%     We elaborate on the extra $q$ fraction of cost. In the worst case scenario, we need an integral from the $r$-far region to an original sample, and solve for the following integration
%     \begin{equation*}
%         \int_{0}^{d_q} p(\|x_{t} - x_0\| = r - s; \sigma^2) (2 s) d s = q \cdot C_{OT}
%     \end{equation*}
%     to get $d_q$, which means for those noisy sample purification that we had additional cost, these purification used the minimum additional cost to get the wrong purification outcome (the 1-D case actually provides an upper bound, meaning that in high dimensional space, to get wrong purification for samples in $[r-d_q, r)$ distance to the original sample, the additional cost is higher than $\int_{0}^{d_q} p(\|x_{t} - x_0\| = r - s; \sigma^2) (2 s) d s$, since the distance to the wrong sample is larger than $r+x$ due to triangle inequality). Consequently, the purification error rate becomes $p_{\mathcal{D},\sigma^2_t} + \int_{0}^{d_q} p(\|x_{t} - x_0\| = r - s; \sigma^2) d s$.
% \end{proof}
% We note that $h(q;\sigma^2_t)$ bounds the additional purification error of the denoiser's deviation from the OT-ODE, and choosing better baselines than the OT-ODE to reduce the inevitable $p_{\mathcal{D},\sigma^2_t}$ remains an interesting future direction.

% \zz{The neighbourhood above actually is quite coarse and especially, it does not show that the distance between the denoised sample and the true sample is smaller than the distance between the adversarial sample and the true sample. However, it maybe possible that there is a contraction area around each true sample for \ref{EDMODE}. The advantage of ODE over SDE in this case is that ODE is deterministic and we do not have to rely on majority vote to locate the denoised sample.}


% \textbf{Theorem Overview for advantages of FT}

% \begin{itemize}
%     \item \textbf{Characterization of Optimal Transport:} Map a noised sample to the nearest data point under the assumption of a discrete original distribution. An ideal mapping aims to approximate the optimal transport within a defined margin of error.

%     \item \textbf{Inter-class Distance Assumption:} Suppose the distance between any two data points from different classes is at least \(d = 2r\). This constraint may be relaxed with a certain probability, accommodating the inherent variability in practical datasets.

%     \item \textbf{Denoiser Efficacy:} If the denoiser maps the noised sample to the data manifold, and the induced transport cost by this mapping is \((1+x)\%\) of the optimal transport cost between the noisy and original distributions, then, with at least probability \(p\), the denoiser will correctly classify the noised sample into the same class as the true sample. The probability of this correct classification $p$ depends on the distance $r$ between the noised and true samples, which can be modeled using a chi-square distribution. It would be beneficial to include a numerical presentation for this model on the CIFAR-10 dataset, showing, for example, that for a \(p\)-value of 0.05, the corresponding radius \(r\) is smaller than \(d\).

%     \item \textbf{Simplification for Practical Application:} In reality, the denoiser may not exactly map the noised sample back to the data manifold but rather to a neighborhood close to it. This effect is acknowledged but not quantified in the current analysis for simplicity.
% \end{itemize}

